Graph Optimal Transport for Cross-Domain Alignment

Cross-domain alignment between two sets of entities (e.g., objects in an image, words in a sentence) is fundamental to both computer vision and natural language processing. Existing methods mainly focus on designing advanced attention mechanisms to simulate soft alignment, with no training signals to explicitly encourage alignment. The learned attention matrices are also dense and lacks interpretability. We propose Graph Optimal Transport (GOT), a principled framework that germinates from recent advances in Optimal Transport (OT). In GOT, cross-domain alignment is formulated as a graph matching problem, by representing entities into a dynamically-constructed graph. Two types of OT distances are considered: (i) Wasserstein distance (WD) for node (entity) matching; and (ii) Gromov-Wasserstein distance (GWD) for edge (structure) matching. Both WD and GWD can be incorporated into existing neural network models, effectively acting as a drop-in regularizer. The inferred transport plan also yields sparse and self-normalized alignment, enhancing the interpretability of the learned model. Experiments show consistent outperformance of GOT over baselines across a wide range of tasks, including image-text retrieval, visual question answering, image captioning, machine translation, and text summarization.

==> ICML2020_ Graph Optimal Transport/alg/gotd_alg.tex <==
\begin{algorithm}[!h]
\caption{Computing GOT Distance.}
\label{alg:gotd}
\begin{algorithmic}[1]
\STATE {\bfseries Input:} \footnotesize{ $\{\xv_i\}_{i=1}^n$,$\{\yv_j\}_{j=1}^m$}, hyper-parameter $\lambda$
\STATE Compute intra-domain similarities:
\STATE
\quad $[\Cmat_x]_{ij} = \cos(\xv_i, \xv_j)$, $[\Cmat_y]_{ij} = \cos(\yv_i, \yv_j)$,
\STATE $\xv'_i=g_1(\xv_i)$, $\yv'_j=g_2(\yv_j)$ // $g_1, g_2$ denote two MLPs
\STATE Compute cross-domain similarities:
\STATE \quad $\Cmat_{ij} = \cos(\xv'_i, \yv'_j)$
\IF{ $\Tmat$ is shared:}
    \STATE Update $\Lcal$ in Algorithm 2 (Line 8) with:
    \STATE \quad $\Lcal_{\text{unified}}=\lambda \Cmat + (1-\lambda) \Lcal $
    \STATE Plug in $\Lcal_{\text{unified}}$ back to Algorithm 2 and solve new $\Tmat$
    % \STATE Using the shared $\Tmat$, calculate $\mathcal{D}_{w}$ and $\mathcal{D}_{gw}$:
    \STATE Compute $\mathcal{D}_{got}$ 
    %via Eqn. (\ref{eq:gotd}).
\ELSE 
    \STATE Apply Algorithm 1 to obtain $\mathcal{D}_{w}$
    \STATE Apply Algorithm 2 to obtain $\mathcal{D}_{gw}$
    \STATE $\mathcal{D}_{got} = \lambda \mathcal{D}_{w} + (1-\lambda) \mathcal{D}_{gw}$
\ENDIF
\STATE Return $\mathcal{D}_{got}$
% \ELSE ddd
\end{algorithmic}
\end{algorithm}

==> ICML2020_ Graph Optimal Transport/alg/gwd_alg.tex <==
\begin{algorithm}[!t]
\caption{Computing Gromov-Wasserstein Distance.}
\label{alg:gwd}
\begin{algorithmic}[1]
% batch size $n$,
\STATE {\bfseries Input:} \footnotesize{ $\{\xv_i\}_{i=1}^n$,$\{\yv_j\}_{j=1}^n$, probability vectors $\pv$, $\qv$} 

\STATE Compute intra-domain similarities:
\STATE
\quad $[\Cmat_{x}]_{ij} = \cos(\xv_i, \xv_j)$, $[\Cmat_{y}]_{ij} = \cos(\yv_i, \yv_j)$,
\STATE Compute cross-domain similarities:
\STATE \quad $\Cmat_{xy} = \Cmat_x^2 \pv \mathbf{1_m}^\top + \Cmat_y \qv (\Cmat_y^2)^\top$
\FOR{$t=1,2,3\ldots$}
    \STATE // Compute the pseudo-cost matrix
    \STATE $\Lcal = \Cmat_{xy} - 2\Cmat_x \Tmat \Cmat_y^\top$
    \STATE Apply Algorithm \ref{alg:wd} to solve transport plan $\Tmat$ 
\ENDFOR
\STATE $\mathcal{D}_{gw}=\langle \Lcal^{\top}, \Tmat\rangle$ \STATE Return $\Tmat$, $\mathcal{D}_{gw}$
% \footnotesize{// $\odot$ is Hadamard product}
% // \footnotesize{$\langle \cdot, \cdot \rangle$ is the Frobenius dot-product} 
\end{algorithmic}
\end{algorithm}

==> ICML2020_ Graph Optimal Transport/alg/wd_alg.tex <==
\begin{algorithm}[!t]
\caption{Computing Wasserstein Distance.}
\label{alg:wd}
\begin{algorithmic}[1]
% batch size $n$,
\STATE {\bfseries Input:} \footnotesize{ $\{\xv_i\}_{i=1}^n$,$\{\yv_j\}_{j=1}^n$, $\beta$}
\STATE $\boldsymbol{\sigma}=\frac{1}{n}\mathbf{1_n}$, $\Tmat^{(1)} = \mathbf{1} \mathbf{1}^\top$
\STATE $\Cmat_{ij} = c(\xv_i, \yv_j)$, $\Amat_{ij} = {\rm e}^{-\frac{\Cmat_{ij}}{\beta}}$
\FOR{$t=1,2,3\ldots$}
    \STATE $\Qmat = \Amat \odot \Tmat^{(t)}$ \footnotesize{// $\odot$ is Hadamard product}
    \FOR{$k=1,2,3,\ldots K$}
        \STATE $\boldsymbol{\delta} = \frac{1}{n\Qmat{\boldsymbol{\sigma}}}$, $\boldsymbol{\sigma} = \frac{1}{n\Qmat^\top\boldsymbol{\delta}}$
    \ENDFOR
    \STATE $\Tmat^{(t+1)} = \text{diag}(\boldsymbol{\delta})\Qmat\text{diag}(\boldsymbol{\sigma})$
\ENDFOR
\STATE $\mathcal{D}_{wd}=\langle \Cmat^{\top}, \Tmat\rangle$ 
\STATE Return $\Tmat$, $\mathcal{D}_{w}$
% \footnotesize{// $\odot$ is Hadamard product}
// \footnotesize{$\langle \cdot, \cdot \rangle$ is the Frobenius dot-product} 
\end{algorithmic}
\end{algorithm}

==> ICML2020_ Graph Optimal Transport/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


\newcommand{\Amat}{{\bf A}}
\newcommand{\Bmat}{{\bf B}}
\newcommand{\Cmat}{{\bf C}}
\newcommand{\Dmat}{{\bf D}}
\newcommand{\Emat}{{\bf E}}
\newcommand{\Fmat}{{\bf F}}
\newcommand{\Gmat}{{\bf G}}
\newcommand{\Hmat}{{\bf H}}
\newcommand{\Imat}{{\bf I}}
\newcommand{\Jmat}{{\bf J}}
\newcommand{\Kmat}{{\bf K}}
\newcommand{\Lmat}{{\bf L}}
\newcommand{\Mmat}{{\bf M}}
\newcommand{\Nmat}{{\bf N}}
\newcommand{\Omat}{{\bf O}}
\newcommand{\Pmat}{{\bf P}}
\newcommand{\Qmat}{{\bf Q}}
\newcommand{\Rmat}{{\bf R}}
\newcommand{\Smat}{{\bf S}}
\newcommand{\Tmat}{{\bf T}}
\newcommand{\Umat}{{\bf U}}
\newcommand{\Vmat}{{\bf V}}
\newcommand{\Wmat}{{\bf W}}
\newcommand{\Xmat}{{\bf X}}
\newcommand{\Ymat}{{\bf Y}}
\newcommand{\Zmat}{{\bf Z}}

\newcommand{\av}{{\boldsymbol a}}
\newcommand{\Av}{{\boldsymbol A}}
\newcommand{\Cv}{{\boldsymbol C}}
\newcommand{\bv}{{\boldsymbol b}}
\newcommand{\cv}{{\boldsymbol c}}
\newcommand{\dv}{{\boldsymbol d}}
\newcommand{\ev}{{\boldsymbol e}}
\newcommand{\fv}{{\boldsymbol f}}
\newcommand{\Fv}{{\boldsymbol F}}
\newcommand{\gv}{{\boldsymbol g}}
\newcommand{\hv}{{\boldsymbol h}}
\newcommand{\iv}{{\boldsymbol i}}
\newcommand{\jv}{{\boldsymbol j}}
\newcommand{\kv}{{\boldsymbol k}}
\newcommand{\lv}{{\boldsymbol l}}
\newcommand{\mv}{{\boldsymbol m}}
\newcommand{\nv}{{\boldsymbol n}}
\newcommand{\ov}{{\boldsymbol o}}
\newcommand{\pv}{{\boldsymbol p}}
\newcommand{\qv}{{\boldsymbol q}}
\newcommand{\rvvv}{{\boldsymbol r}}
\newcommand{\sv}{{\boldsymbol s}}
\newcommand{\tv}{{\boldsymbol t}}
\newcommand{\uv}{{\boldsymbol u}}
\newcommand{\vvv}{{\boldsymbol v}}
\newcommand{\wv}{{\boldsymbol w}}
\newcommand{\Wv}{{\boldsymbol W}}
\newcommand{\xv}{{\boldsymbol x}}
\newcommand{\yv}{{\boldsymbol y}}
\newcommand{\Xv}{{\boldsymbol X}}
\newcommand{\Yv}{{\boldsymbol Y}}
\newcommand{\zv}{{\boldsymbol z}}

\newcommand{\Gammamat}{{\boldsymbol \Gamma}}
\newcommand{\Deltamat}{{\boldsymbol \Delta}}
\newcommand{\Thetamat}{{\boldsymbol \Theta}}
\newcommand{\Ximat}{{\boldsymbol \Xi}}
\newcommand{\Pimat}{{\boldsymbol \Pi}}
\newcommand{\Sigmamat}{{\boldsymbol \Sigma}}
\newcommand{\Upsilonmat}{{\boldsymbol \Upsilon}}
\newcommand{\Phimat}{{\boldsymbol \Phi}}
\newcommand{\Psimat}{{\boldsymbol \Psi}}
\newcommand{\Omegamat}{{\boldsymbol \Omega}}
\newcommand{\Lambdamat}{{\boldsymbol \Lambda}}
\newcommand{\zerov}{{\boldsymbol 0}}

\newcommand{\alphav}{{\boldsymbol \alpha}}
\newcommand{\betav}{{\boldsymbol \beta}}
\newcommand{\gammav}{{\boldsymbol \gamma}}
\newcommand{\deltav}{{\boldsymbol \delta}}
\newcommand{\epsilonv}{{\boldsymbol \epsilon}}
\newcommand{\zetav}{{\boldsymbol \zeta}}
\newcommand{\etav}{{\boldsymbol \eta}}
\newcommand{\thetav}{{\boldsymbol \theta}}
\newcommand{\iotav}{{\boldsymbol \iota}}
\newcommand{\kappav}{{\boldsymbol \kappa}}
\newcommand{\lambdav}{{\boldsymbol \lambda}}
\newcommand{\muv}{{\boldsymbol \mu}}
\newcommand{\nuv}{{\boldsymbol \nu}}
\newcommand{\xiv}{{\boldsymbol \xi}}
\newcommand{\omicronv}{{\boldsymbol \omicron}}
\newcommand{\piv}{{\boldsymbol \pi}}
\newcommand{\rhov}{{\boldsymbol \rho}}
\newcommand{\sigmav}{{\boldsymbol \sigma}}
\newcommand{\tauv}{{\boldsymbol \tau}}
\newcommand{\upsilonv}{{\boldsymbol \upsilon}}
\newcommand{\phiv}{{\boldsymbol \phi}}
\newcommand{\chiv}{{\boldsymbol \chi}}
\newcommand{\psiv}{{\boldsymbol \psi}}
\newcommand{\omegav}{{\boldsymbol \omega}}


\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\NNcal}{\mathcal{N}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Rcal}{\mathcal{R}}

\newtheorem{theorem}{Theorem}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}



==> ICML2020_ Graph Optimal Transport/table/abs_sum.tex <==
\begin{table}[t!]
    \centering
    \small
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{l c c c} %{L{5.5cm} l}
    \hline
    {\bf Method} & {\bf ROUGE-1} & {\bf ROUGE-2} & {\bf ROUGE-L}\\ 
    \hline
    ABS+~\cite{rush2015neural} & $31.00$  & $12.65$ & $28.34$ \\
    LSTM~\cite{hu2018texar} & $36.11 $ & $16.39 $ & $32.32 $ \\
    LSTM + GWD  & $36.31 $ & $17.32 $ & $33.15 $ \\
    LSTM + WD  & $36.81 $ & $17.34 $ & $33.34 $ \\
    LSTM + GOT & \bm{$37.10$} & \bm{$17.61 $} & \bm{$33.70 $} \\
    % LSTM \cite{seq2seq} & $36.11 \pm 0.21$ & $16.39 \pm 0.16$ & $32.32 \pm 0.19$ \\
    % LSTM + GWD  & $36.31 \pm 0.25$ & $17.32 \pm 0.16$ & $33.15 \pm 0.23$ \\
    % LSTM + WD  & $36.81 \pm 0.25$ & $17.34 \pm 0.16$ & $33.34 \pm 0.23$ \\
    % \textbf{Ours}: LSTM + GOT & \bm{$37.1 \pm 0.19$} & \bm{$17.61 \pm 0.15$} & \bm{$33.70 \pm 0.13$} \\
    \hline
    \end{tabular}
    }
    \vspace{-2mm}
    \caption{\label{tab:giga} Results of abstractive text summarization on the English Gigawords dataset.}
    %\vspace{-3mm}
\end{table}

==> ICML2020_ Graph Optimal Transport/table/ban_vqa_ablation.tex <==
\begin{table}[!t]
    \centering
    \small
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{l c c c c c} %{L{5.5cm} l}
    \hline
    {\bf Model}  & {\bf BUTD} & {\bf BAN-1} & {\bf BAN-2} & {\bf BAN-4} & {\bf BAN-8}\\ 
    \hline
    {\bf w/o GOT }  & 63.37 & 65.37 & 65.61 & 65.81 & 66.00 \\
    {\bf w/ GOT } & \textbf{65.01} & \textbf{65.68} & \textbf{65.88} & \textbf{66.10} & \textbf{66.44} \\
    \hline
    \end{tabular}
    }
    \vspace{-3mm}
    \caption{\label{tab:vqa_dfBAN} Results (accuracy) of applying GOT to BUTD~\cite{anderson2018bottom} and BAN-$m$~\cite{kim2018bilinear} on VQA 2.0. $m$ denotes the number of glimpses.}
    %\vspace{-2mm}
\end{table}

==> ICML2020_ Graph Optimal Transport/table/imageCaption.tex <==
\begin{table*}[ht!]\small
    \centering
\resizebox{0.92\textwidth}{!}{
\begin{tabular}{lccccccc}
\hline
Method           & CIDEr & BLEU-4 & BLUE-3 & BLEU-2 & BLEU-1 & ROUGE & METEOR \\ \hline
%DeepVS~\citep{karpathy2015deep}  &    62.5 & 45.0 & 32.1 & 23.0 & 19.5 & 66.0 \\
Soft Attention~\citep{xu2015show}  & - & 24.3 & 34.4 & 49.2 & 70.7 & - &23.9\\
Hard Attention~\citep{xu2015show}  &  - & 25.0 & 35.7 & 50.4 & 71.8 & -&23.0 \\
Show \& Tell~\citep{vinyals2015show} & 85.5 & 27.7    & -    & - & - & -& 23.7 \\
ATT-FCN~\citep{you2016image} &    - & 30.4 & 40.2 & 53.7 & 70.9 & - & 24.3\\
SCN-LSTM~\citep{gan2017semantic} & 101.2 & 33.0 & 43.3 & 56.6 & 72.8 & -& 25.7\\
Adaptive Attention~\citep{lu2017knowing}  &  108.5 & 33.2 & 43.9 &  58.0 &  74.2 & -& 26.6 \\
\hline
MLE              & 106.3 & 34.3   & 45.3   & 59.3   & 75.6   & 55.2  & 26.2   \\
MLE + WD        & 107.9 & {34.8}   & 46.1   & 60.1   & 76.2   & 55.6  & 26.5   \\
MLE + GWD          & 106.6 & {33.3}   & 45.2   & 59.1   & 75.7   & 55.0  & 25.9   \\
MLE + GOT  & \textbf{109.2} & \textbf{35.1}   & \textbf{46.5}   & \textbf{60.3}   & \textbf{77.0}   & \textbf{56.2}  & \textbf{26.7}   \\ \hline
\end{tabular}}
\caption{ \label{table:caption}Results of image captioning on the COCO dataset. }
%\vspace{-2mm}
\end{table*}

==> ICML2020_ Graph Optimal Transport/table/retrieval.tex <==
\begin{table*}[t!]
  \begin{center}
  \centering
  \small
    % \begin{tabular}{lccccccc}
    \begin{tabular*}{1.\linewidth}{@{\extracolsep{\fill}}lccccccc}
         \toprule
        %  \noalign{\smallskip}
         & \multicolumn{3}{c}{Sentence Retrieval} & \multicolumn{3}{c}{Image Retrieval} & \multicolumn{1}{c}{}\\
        Method & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 &Rsum\\
        % \noalign{\smallskip}
        \toprule
        % \noalign{\smallskip}
        % & \multicolumn{7}{c}{Flickr30K} \\ 
        % \hline
        % \noalign{\smallskip}
        % DVSA (R-CNN, AlexNet) \cite{karpathy2015deep} & 22.2 & 48.2 & 61.4 & 15.2 & 37.7 & 50.5 & 235.2\\ 
        % HM-LSTM (R-CNN, AlexNet) \cite{niu2017hierarchical} & 38.1 & -- & 76.5 & 27.7 & -- & 68.8 & --\\ 
        % DSPE (VGG) \cite{wang2016learning} & 40.3 & 68.9 & 79.9 & 29.7 & 60.1 & 72.1 \\ 
        % 2WayNet (VGG) \cite{eisenschtat2017linking} & 49.8 & 67.5 & -- & 36.0 & 55.6 & -- & --\\ 
        % SM-LSTM (VGG) \cite{huang2017instance} & 42.5 & 71.9 & 81.5 & 30.2 & 60.4 & 72.3 & 358.8\\ 
        VSE++ (ResNet) \cite{VSE} & 52.9 & -- & 87.2 & 39.6 & -- & 79.5 & -- \\ 
        DPC (ResNet) \cite{zheng2017dual} & 55.6 & 81.9 & 89.5 & 39.1 & 69.2 & 80.9 & 416.2\\ 
        DAN (ResNet) \cite{nam2017dual} & 55.0 & 81.8 & 89.0 & 39.4 & 69.2 & 79.1 & 413.5\\ 
        SCO (ResNet) \cite{huang2018learning} & 55.5 & 82.0 & 89.3 & 41.1 & 70.5 & 80.1 & 418.5\\ 
        SCAN (Faster R-CNN, ResNet) \cite{SCAN}  & 67.7 & 88.9 & 94.0 & 44.0 & 74.2 & 82.6 &452.2 \\ 
        \textbf{Ours (Faster R-CNN, ResNet)}:\\
        SCAN + WD  &{70.9} &{92.3} &{95.2} &{49.7} &{ 78.2} &{86.0} &{472.3
}\\
        SCAN + GWD  &{69.5} &{91.2} &{95.2} &{48.8} &{78.1} &{85.8} &{468.6}\\
        SCAN + GOT  &\textbf{70.9} &\textbf{92.8} &\textbf{95.5} &\textbf{50.7} & \textbf{78.7} &\textbf{86.2} &\textbf{474.8}\\
        % $\cos$ + OT (Ensemble model) &\textbf{69.3} &\textbf{91.6} &{95.1} &\textbf{49.8} &\textbf{78.1} &\textbf{85.6} &\textbf{469.5}\\
        % $\cos$ + OT (Ensemble) &{69.0} &{90.7} &{95.7} &\textbf{50.1} &\textbf{78.4} &\textbf{85.6} &\textbf{469.5}\\
        % \hline
        % \hline
        \hline
        \noalign{\smallskip}
        % & \multicolumn{7}{c}{MS-COCO} \\ 
        % \midrule
        % \hline
        % Order-embeddings (VGG) \cite{vendrov2015order} & 23.3 & -- & 84.7 & 31.7 & -- & 74.6 & -- \\ 
        VSE++ (ResNet) \cite{VSE} & 41.3 & -- & 81.2 & 30.3 & -- & 72.4 & -- \\ 
        DPC (ResNet) \cite{zheng2017dual} & 41.2 & 70.5 & 81.1 & 25.3 & 53.4 & 66.4 & 337.9\\ 
        GXN (ResNet) \cite{gu2018look} & 42.0 & -- & 84.7 & 31.7 & -- & 74.6 & -- \\ 
        SCO (ResNet) \cite{huang2018learning} & 42.8 & 72.3 & 83.0 & 33.1 & 62.9 & 75.5 & 369.6 \\ 
        SCAN (Faster R-CNN, ResNet)\cite{SCAN} & 46.4 & 77.4 & 87.2 & 34.4 & 63.7 & 75.7 & 384.8 \\ 
        % SCAN (Ensemble)\cite{SCAN} & {50.4} & {82.2} & {90.0} & {38.6} & {69.3} & {80.4} & 410.9 \\ 
        % \hline
        \textbf{Ours (Faster R-CNN, ResNet)}:\\
        SCAN + WD &{50.2} &{80.1} &{89.5} &{37.9} &{66.8} &{78.1} &{402.6}\\
        SCAN + GWD &{47.2} & {78.3} &{87.5} &{34.9} &{64.4} &{76.3} &{388.6
}\\
        SCAN + GOT &\textbf{50.5} &\textbf{80.2} &\textbf{89.8} &\textbf{38.1} & \textbf{66.8} &\textbf{78.5} &\textbf{403.9}\\
        %$\cos$ + OT (Ensemble) &\textbf{52.1} &\textbf{82.4} &\textbf{90.7} &\textbf{39.1} &{68.2} &{79.2} &\textbf{411.7}\\
        % Dot + OT (single model, m=0.12) &\textbf{69.3} &{91.0} &{95.7} &{48.4} &{77.2} &{84.7} &{466.3}\\
        % Dot + OT (ensembled model) &\textbf{69.3} &\textbf{91.6} &{95.1} &\textbf{49.8} &\textbf{78.1} &\textbf{85.6} &\textbf{469.5}\\
        \bottomrule
    \end{tabular*}
    \vspace{-2mm}
     \caption{\label{table:retrieval} Results on image-text retrieval evaluated on Recall@$K$ (R@$K$). Upper panel: Flickr30K; lower panel: COCO. 
  }
    \vspace{-3mm}
  \end{center}
\end{table*}

==> ICML2020_ Graph Optimal Transport/table/translate.tex <==

\begin{table*}[!t]
    \centering
    \small
    % \resizebox{\textwidth}{!}{
    \begin{tabular}{l c c c c} %{L{5.5cm} l}
    \hline
    {\bf Model}  & {\bf EN-VI uncased} & {\bf EN-VI cased} & {\bf EN-DE uncased} & {\bf EN-DE cased}\\ 
    \hline
    Transformer~\cite{vaswani2017attention}    & $29.25 \pm 0.18$ & $28.46 \pm 0.17$ & $25.60 \pm 0.07$ & $25.12 \pm 0.12$\\
    Transformer + WD  & $29.49 \pm 0.10$ & $28.68 \pm 0.14$ & $25.83 \pm 0.12$ & $25.30 \pm 0.11$\\
    Transformer + GWD & $28.65 \pm 0.14$ & $28.34 \pm 0.16$ & $25.42 \pm 0.17$ & $24.82 \pm 0.15$\\
    Transformer + GOT & $\mathbf{29.92 \pm 0.11}$ & $\mathbf{29.09 \pm 0.18}$ & $\mathbf{26.05 \pm 0.17}$ & $\mathbf{25.54 \pm 0.15}$\\
    \hline
    \end{tabular}
    % }
    \vspace{-2mm}
    \caption{\label{tab:mt} Results of neural machine translation on EN-DE and EN-VI.}
    %\vspace{-3mm}
\end{table*}


==> ICML2020_ Graph Optimal Transport/table/translate_ablation.tex <==

\begin{table}[t]
    \centering
    \small
    % \resizebox{\textwidth}{!}{
    \begin{tabular}{l c c } %{L{5.5cm} l}
    \hline
    {\bf Model}  & {\bf EN-VI uncased} & {\bf EN-DE uncased} \\ 
    \hline
    GOT (shared) & ${29.92 \pm 0.11}$ & ${26.05 \pm 0.18}$  \\
    GOT (unshared) & ${29.77 \pm 0.12}$ & ${25.89 \pm 0.17}$  \\
    \hline
    \end{tabular}
    % }
    \caption{\label{tab:mt_ablation_shareT} Ablation study on transport plan in machine translation. Both models were run 5 times with the same hyper-parameter setting.}
\end{table}


==> ICML2020_ Graph Optimal Transport/table/translate_lambda_ablation.tex <==

%\begin{table}[!t]
%    \centering
%    \small
%%    %\resizebox{0.48\textwidth}{!}{
%    \begin{tabular}{l c c c c c} %{L{5.5cm} l}
%    \hline
%    {\bf Model}  & {\bf BUTD} & {\bf BAN} & {\bf BAN+GW} & {\bf BAN+W} & {\bf BAN+GOT}\\ 
%    \hline
%    
%    {\bf Score} & $63.37$ & $66.00$ & $66.21$ & $66.26$ & $66.44$\\
%
%    \hline
%    \end{tabular}
%    %}
%    \caption{\label{tab:vqa} Results on VQA 2.0 validation set. \cite{kim2018bilinear}}
%    \vspace{-3mm}
%\end{table}

\begin{table}[!t]
    \centering
    \small
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{l c  c c c c c} %{L{5.5cm} l}
    \hline
    {\bf $\lambda$}  & 0  & 0.1 & 0.3 & 0.5 & 0.8 & 1.0\\ 
    \hline
    
    {\bf BLEU} & $28.65$  & $29.31$ & $29.52$ & $29.65$ & {\bf 29.92} & $29.49$\\

    \hline
    \end{tabular}
    }
    \vspace{-3mm}
    \caption{\label{tab:lambda_ab} Ablation study of the hyper-parameter $\lambda$ on the EN-VI machine translation dataset.}
    \vspace{-3mm}
\end{table}


==> ICML2020_ Graph Optimal Transport/table/vqa_ban.tex <==

%\begin{table}[!t]
%    \centering
%    \small
%%    %\resizebox{0.48\textwidth}{!}{
%    \begin{tabular}{l c c c c c} %{L{5.5cm} l}
%    \hline
%    {\bf Model}  & {\bf BUTD} & {\bf BAN} & {\bf BAN+GW} & {\bf BAN+W} & {\bf BAN+GOT}\\ 
%    \hline
%    
%    {\bf Score} & $63.37$ & $66.00$ & $66.21$ & $66.26$ & $66.44$\\
%
%    \hline
%    \end{tabular}
%    %}
%    \caption{\label{tab:vqa} Results on VQA 2.0 validation set. \cite{kim2018bilinear}}
%    \vspace{-3mm}
%\end{table}

\begin{table}[!t]
    \centering
    \small
    %\resizebox{0.48\textwidth}{!}{
    \begin{tabular}{l c c c c} %{L{5.5cm} l}
    \hline
    {\bf Model}  &  {\bf BAN} & {\bf BAN+GWD} & {\bf BAN+WD} & {\bf BAN+GOT}\\ 
    \hline
    
    {\bf Score} & 66.00 & 66.21 & 66.26 & \textbf{66.44}\\

    \hline
    \end{tabular}
    %}
    \vspace{-3mm}
    \caption{\label{tab:vqa} Results (accuracy) on VQA 2.0 validation set, using BAN~\cite{kim2018bilinear} as baseline.}
    %\vspace{-2mm}
\end{table}


==> alg/gotd_alg.tex <==
\begin{algorithm}[!h]
\caption{Computing GOT Distance.}
\label{alg:gotd}
\begin{algorithmic}[1]
\STATE {\bfseries Input:} \footnotesize{ $\{\xv_i\}_{i=1}^n$,$\{\yv_j\}_{j=1}^m$}, hyper-parameter $\lambda$
\STATE Compute intra-domain similarities:
\STATE
\quad $[\Cmat_x]_{ij} = \cos(\xv_i, \xv_j)$, $[\Cmat_y]_{ij} = \cos(\yv_i, \yv_j)$,
\STATE $\xv'_i=g_1(\xv_i)$, $\yv'_j=g_2(\yv_j)$ // $g_1, g_2$ denote two MLPs
\STATE Compute cross-domain similarities:
\STATE \quad $\Cmat_{ij} = \cos(\xv'_i, \yv'_j)$
\IF{ $\Tmat$ is shared:}
    \STATE Update $\Lcal$ in Algorithm 2 (Line 8) with:
    \STATE \quad $\Lcal_{\text{unified}}=\lambda \Cmat + (1-\lambda) \Lcal $
    \STATE Plug in $\Lcal_{\text{unified}}$ back to Algorithm 2 and solve new $\Tmat$
    % \STATE Using the shared $\Tmat$, calculate $\mathcal{D}_{w}$ and $\mathcal{D}_{gw}$:
    \STATE Compute $\mathcal{D}_{got}$ 
    %via Eqn. (\ref{eq:gotd}).
\ELSE 
    \STATE Apply Algorithm 1 to obtain $\mathcal{D}_{w}$
    \STATE Apply Algorithm 2 to obtain $\mathcal{D}_{gw}$
    \STATE $\mathcal{D}_{got} = \lambda \mathcal{D}_{w} + (1-\lambda) \mathcal{D}_{gw}$
\ENDIF
\STATE Return $\mathcal{D}_{got}$
% \ELSE ddd
\end{algorithmic}
\end{algorithm}

==> alg/gwd_alg.tex <==
\begin{algorithm}[!t]
\caption{Computing Gromov-Wasserstein Distance.}
\label{alg:gwd}
\begin{algorithmic}[1]
% batch size $n$,
\STATE {\bfseries Input:} \footnotesize{ $\{\xv_i\}_{i=1}^n$,$\{\yv_j\}_{j=1}^n$, probability vectors $\pv$, $\qv$} 

\STATE Compute intra-domain similarities:
\STATE
\quad $[\Cmat_{x}]_{ij} = \cos(\xv_i, \xv_j)$, $[\Cmat_{y}]_{ij} = \cos(\yv_i, \yv_j)$,
\STATE Compute cross-domain similarities:
\STATE \quad $\Cmat_{xy} = \Cmat_x^2 \pv \mathbf{1_m}^\top + \Cmat_y \qv (\Cmat_y^2)^\top$
\FOR{$t=1,2,3\ldots$}
    \STATE // Compute the pseudo-cost matrix
    \STATE $\Lcal = \Cmat_{xy} - 2\Cmat_x \Tmat \Cmat_y^\top$
    \STATE Apply Algorithm \ref{alg:wd} to solve transport plan $\Tmat$ 
\ENDFOR
\STATE $\mathcal{D}_{gw}=\langle \Lcal^{\top}, \Tmat\rangle$ \STATE Return $\Tmat$, $\mathcal{D}_{gw}$
% \footnotesize{// $\odot$ is Hadamard product}
% // \footnotesize{$\langle \cdot, \cdot \rangle$ is the Frobenius dot-product} 
\end{algorithmic}
\end{algorithm}

==> alg/wd_alg.tex <==
\begin{algorithm}[!t]
\caption{Computing Wasserstein Distance.}
\label{alg:wd}
\begin{algorithmic}[1]
% batch size $n$,
\STATE {\bfseries Input:} \footnotesize{ $\{\xv_i\}_{i=1}^n$,$\{\yv_j\}_{j=1}^n$, $\beta$}
\STATE $\boldsymbol{\sigma}=\frac{1}{n}\mathbf{1_n}$, $\Tmat^{(1)} = \mathbf{1} \mathbf{1}^\top$
\STATE $\Cmat_{ij} = c(\xv_i, \yv_j)$, $\Amat_{ij} = {\rm e}^{-\frac{\Cmat_{ij}}{\beta}}$
\FOR{$t=1,2,3\ldots$}
    \STATE $\Qmat = \Amat \odot \Tmat^{(t)}$ \footnotesize{// $\odot$ is Hadamard product}
    \FOR{$k=1,2,3,\ldots K$}
        \STATE $\boldsymbol{\delta} = \frac{1}{n\Qmat{\boldsymbol{\sigma}}}$, $\boldsymbol{\sigma} = \frac{1}{n\Qmat^\top\boldsymbol{\delta}}$
    \ENDFOR
    \STATE $\Tmat^{(t+1)} = \text{diag}(\boldsymbol{\delta})\Qmat\text{diag}(\boldsymbol{\sigma})$
\ENDFOR
\STATE $\mathcal{D}_{wd}=\langle \Cmat^{\top}, \Tmat\rangle$ 
\STATE Return $\Tmat$, $\mathcal{D}_{w}$
% \footnotesize{// $\odot$ is Hadamard product}
// \footnotesize{$\langle \cdot, \cdot \rangle$ is the Frobenius dot-product} 
\end{algorithmic}
\end{algorithm}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


\newcommand{\Amat}{{\bf A}}
\newcommand{\Bmat}{{\bf B}}
\newcommand{\Cmat}{{\bf C}}
\newcommand{\Dmat}{{\bf D}}
\newcommand{\Emat}{{\bf E}}
\newcommand{\Fmat}{{\bf F}}
\newcommand{\Gmat}{{\bf G}}
\newcommand{\Hmat}{{\bf H}}
\newcommand{\Imat}{{\bf I}}
\newcommand{\Jmat}{{\bf J}}
\newcommand{\Kmat}{{\bf K}}
\newcommand{\Lmat}{{\bf L}}
\newcommand{\Mmat}{{\bf M}}
\newcommand{\Nmat}{{\bf N}}
\newcommand{\Omat}{{\bf O}}
\newcommand{\Pmat}{{\bf P}}
\newcommand{\Qmat}{{\bf Q}}
\newcommand{\Rmat}{{\bf R}}
\newcommand{\Smat}{{\bf S}}
\newcommand{\Tmat}{{\bf T}}
\newcommand{\Umat}{{\bf U}}
\newcommand{\Vmat}{{\bf V}}
\newcommand{\Wmat}{{\bf W}}
\newcommand{\Xmat}{{\bf X}}
\newcommand{\Ymat}{{\bf Y}}
\newcommand{\Zmat}{{\bf Z}}

\newcommand{\av}{{\boldsymbol a}}
\newcommand{\Av}{{\boldsymbol A}}
\newcommand{\Cv}{{\boldsymbol C}}
\newcommand{\bv}{{\boldsymbol b}}
\newcommand{\cv}{{\boldsymbol c}}
\newcommand{\dv}{{\boldsymbol d}}
\newcommand{\ev}{{\boldsymbol e}}
\newcommand{\fv}{{\boldsymbol f}}
\newcommand{\Fv}{{\boldsymbol F}}
\newcommand{\gv}{{\boldsymbol g}}
\newcommand{\hv}{{\boldsymbol h}}
\newcommand{\iv}{{\boldsymbol i}}
\newcommand{\jv}{{\boldsymbol j}}
\newcommand{\kv}{{\boldsymbol k}}
\newcommand{\lv}{{\boldsymbol l}}
\newcommand{\mv}{{\boldsymbol m}}
\newcommand{\nv}{{\boldsymbol n}}
\newcommand{\ov}{{\boldsymbol o}}
\newcommand{\pv}{{\boldsymbol p}}
\newcommand{\qv}{{\boldsymbol q}}
\newcommand{\rvvv}{{\boldsymbol r}}
\newcommand{\sv}{{\boldsymbol s}}
\newcommand{\tv}{{\boldsymbol t}}
\newcommand{\uv}{{\boldsymbol u}}
\newcommand{\vvv}{{\boldsymbol v}}
\newcommand{\wv}{{\boldsymbol w}}
\newcommand{\Wv}{{\boldsymbol W}}
\newcommand{\xv}{{\boldsymbol x}}
\newcommand{\yv}{{\boldsymbol y}}
\newcommand{\Xv}{{\boldsymbol X}}
\newcommand{\Yv}{{\boldsymbol Y}}
\newcommand{\zv}{{\boldsymbol z}}

\newcommand{\Gammamat}{{\boldsymbol \Gamma}}
\newcommand{\Deltamat}{{\boldsymbol \Delta}}
\newcommand{\Thetamat}{{\boldsymbol \Theta}}
\newcommand{\Ximat}{{\boldsymbol \Xi}}
\newcommand{\Pimat}{{\boldsymbol \Pi}}
\newcommand{\Sigmamat}{{\boldsymbol \Sigma}}
\newcommand{\Upsilonmat}{{\boldsymbol \Upsilon}}
\newcommand{\Phimat}{{\boldsymbol \Phi}}
\newcommand{\Psimat}{{\boldsymbol \Psi}}
\newcommand{\Omegamat}{{\boldsymbol \Omega}}
\newcommand{\Lambdamat}{{\boldsymbol \Lambda}}
\newcommand{\zerov}{{\boldsymbol 0}}

\newcommand{\alphav}{{\boldsymbol \alpha}}
\newcommand{\betav}{{\boldsymbol \beta}}
\newcommand{\gammav}{{\boldsymbol \gamma}}
\newcommand{\deltav}{{\boldsymbol \delta}}
\newcommand{\epsilonv}{{\boldsymbol \epsilon}}
\newcommand{\zetav}{{\boldsymbol \zeta}}
\newcommand{\etav}{{\boldsymbol \eta}}
\newcommand{\thetav}{{\boldsymbol \theta}}
\newcommand{\iotav}{{\boldsymbol \iota}}
\newcommand{\kappav}{{\boldsymbol \kappa}}
\newcommand{\lambdav}{{\boldsymbol \lambda}}
\newcommand{\muv}{{\boldsymbol \mu}}
\newcommand{\nuv}{{\boldsymbol \nu}}
\newcommand{\xiv}{{\boldsymbol \xi}}
\newcommand{\omicronv}{{\boldsymbol \omicron}}
\newcommand{\piv}{{\boldsymbol \pi}}
\newcommand{\rhov}{{\boldsymbol \rho}}
\newcommand{\sigmav}{{\boldsymbol \sigma}}
\newcommand{\tauv}{{\boldsymbol \tau}}
\newcommand{\upsilonv}{{\boldsymbol \upsilon}}
\newcommand{\phiv}{{\boldsymbol \phi}}
\newcommand{\chiv}{{\boldsymbol \chi}}
\newcommand{\psiv}{{\boldsymbol \psi}}
\newcommand{\omegav}{{\boldsymbol \omega}}


\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\NNcal}{\mathcal{N}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Rcal}{\mathcal{R}}

\newtheorem{theorem}{Theorem}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}



==> table/abs_sum.tex <==
\begin{table}[t!]
    \centering
    \small
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{l c c c} %{L{5.5cm} l}
    \hline
    {\bf Method} & {\bf ROUGE-1} & {\bf ROUGE-2} & {\bf ROUGE-L}\\ 
    \hline
    ABS+~\cite{rush2015neural} & $31.00$  & $12.65$ & $28.34$ \\
    LSTM~\cite{hu2018texar} & $36.11 $ & $16.39 $ & $32.32 $ \\
    LSTM + GWD  & $36.31 $ & $17.32 $ & $33.15 $ \\
    LSTM + WD  & $36.81 $ & $17.34 $ & $33.34 $ \\
    LSTM + GOT & \bm{$37.10$} & \bm{$17.61 $} & \bm{$33.70 $} \\
    % LSTM \cite{seq2seq} & $36.11 \pm 0.21$ & $16.39 \pm 0.16$ & $32.32 \pm 0.19$ \\
    % LSTM + GWD  & $36.31 \pm 0.25$ & $17.32 \pm 0.16$ & $33.15 \pm 0.23$ \\
    % LSTM + WD  & $36.81 \pm 0.25$ & $17.34 \pm 0.16$ & $33.34 \pm 0.23$ \\
    % \textbf{Ours}: LSTM + GOT & \bm{$37.1 \pm 0.19$} & \bm{$17.61 \pm 0.15$} & \bm{$33.70 \pm 0.13$} \\
    \hline
    \end{tabular}
    }
    \vspace{-2mm}
    \caption{\label{tab:giga} Results of abstractive text summarization on the English Gigawords dataset.}
    %\vspace{-3mm}
\end{table}

==> table/ban_vqa_ablation.tex <==
\begin{table}[!t]
    \centering
    \small
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{l c c c c c} %{L{5.5cm} l}
    \hline
    {\bf Model}  & {\bf BUTD} & {\bf BAN-1} & {\bf BAN-2} & {\bf BAN-4} & {\bf BAN-8}\\ 
    \hline
    {\bf w/o GOT }  & 63.37 & 65.37 & 65.61 & 65.81 & 66.00 \\
    {\bf w/ GOT } & \textbf{65.01} & \textbf{65.68} & \textbf{65.88} & \textbf{66.10} & \textbf{66.44} \\
    \hline
    \end{tabular}
    }
    \vspace{-3mm}
    \caption{\label{tab:vqa_dfBAN} Results (accuracy) of applying GOT to BUTD~\cite{anderson2018bottom} and BAN-$m$~\cite{kim2018bilinear} on VQA 2.0. $m$ denotes the number of glimpses.}
    %\vspace{-2mm}
\end{table}

==> table/imageCaption.tex <==
\begin{table*}[ht!]\small
    \centering
\resizebox{0.92\textwidth}{!}{
\begin{tabular}{lccccccc}
\hline
Method           & CIDEr & BLEU-4 & BLUE-3 & BLEU-2 & BLEU-1 & ROUGE & METEOR \\ \hline
%DeepVS~\citep{karpathy2015deep}  &    62.5 & 45.0 & 32.1 & 23.0 & 19.5 & 66.0 \\
Soft Attention~\citep{xu2015show}  & - & 24.3 & 34.4 & 49.2 & 70.7 & - &23.9\\
Hard Attention~\citep{xu2015show}  &  - & 25.0 & 35.7 & 50.4 & 71.8 & -&23.0 \\
Show \& Tell~\citep{vinyals2015show} & 85.5 & 27.7    & -    & - & - & -& 23.7 \\
ATT-FCN~\citep{you2016image} &    - & 30.4 & 40.2 & 53.7 & 70.9 & - & 24.3\\
SCN-LSTM~\citep{gan2017semantic} & 101.2 & 33.0 & 43.3 & 56.6 & 72.8 & -& 25.7\\
Adaptive Attention~\citep{lu2017knowing}  &  108.5 & 33.2 & 43.9 &  58.0 &  74.2 & -& 26.6 \\
\hline
MLE              & 106.3 & 34.3   & 45.3   & 59.3   & 75.6   & 55.2  & 26.2   \\
MLE + WD        & 107.9 & {34.8}   & 46.1   & 60.1   & 76.2   & 55.6  & 26.5   \\
MLE + GWD          & 106.6 & {33.3}   & 45.2   & 59.1   & 75.7   & 55.0  & 25.9   \\
MLE + GOT  & \textbf{109.2} & \textbf{35.1}   & \textbf{46.5}   & \textbf{60.3}   & \textbf{77.0}   & \textbf{56.2}  & \textbf{26.7}   \\ \hline
\end{tabular}}
\caption{ \label{table:caption}Results of image captioning on the COCO dataset. }
%\vspace{-2mm}
\end{table*}

==> table/retrieval.tex <==
\begin{table*}[t!]
  \begin{center}
  \centering
  \small
    % \begin{tabular}{lccccccc}
    \begin{tabular*}{1.\linewidth}{@{\extracolsep{\fill}}lccccccc}
         \toprule
        %  \noalign{\smallskip}
         & \multicolumn{3}{c}{Sentence Retrieval} & \multicolumn{3}{c}{Image Retrieval} & \multicolumn{1}{c}{}\\
        Method & R@1 & R@5 & R@10 & R@1 & R@5 & R@10 &Rsum\\
        % \noalign{\smallskip}
        \toprule
        % \noalign{\smallskip}
        % & \multicolumn{7}{c}{Flickr30K} \\ 
        % \hline
        % \noalign{\smallskip}
        % DVSA (R-CNN, AlexNet) \cite{karpathy2015deep} & 22.2 & 48.2 & 61.4 & 15.2 & 37.7 & 50.5 & 235.2\\ 
        % HM-LSTM (R-CNN, AlexNet) \cite{niu2017hierarchical} & 38.1 & -- & 76.5 & 27.7 & -- & 68.8 & --\\ 
        % DSPE (VGG) \cite{wang2016learning} & 40.3 & 68.9 & 79.9 & 29.7 & 60.1 & 72.1 \\ 
        % 2WayNet (VGG) \cite{eisenschtat2017linking} & 49.8 & 67.5 & -- & 36.0 & 55.6 & -- & --\\ 
        % SM-LSTM (VGG) \cite{huang2017instance} & 42.5 & 71.9 & 81.5 & 30.2 & 60.4 & 72.3 & 358.8\\ 
        VSE++ (ResNet) \cite{VSE} & 52.9 & -- & 87.2 & 39.6 & -- & 79.5 & -- \\ 
        DPC (ResNet) \cite{zheng2017dual} & 55.6 & 81.9 & 89.5 & 39.1 & 69.2 & 80.9 & 416.2\\ 
        DAN (ResNet) \cite{nam2017dual} & 55.0 & 81.8 & 89.0 & 39.4 & 69.2 & 79.1 & 413.5\\ 
        SCO (ResNet) \cite{huang2018learning} & 55.5 & 82.0 & 89.3 & 41.1 & 70.5 & 80.1 & 418.5\\ 
        SCAN (Faster R-CNN, ResNet) \cite{SCAN}  & 67.7 & 88.9 & 94.0 & 44.0 & 74.2 & 82.6 &452.2 \\ 
        \textbf{Ours (Faster R-CNN, ResNet)}:\\
        SCAN + WD  &{70.9} &{92.3} &{95.2} &{49.7} &{ 78.2} &{86.0} &{472.3
}\\
        SCAN + GWD  &{69.5} &{91.2} &{95.2} &{48.8} &{78.1} &{85.8} &{468.6}\\
        SCAN + GOT  &\textbf{70.9} &\textbf{92.8} &\textbf{95.5} &\textbf{50.7} & \textbf{78.7} &\textbf{86.2} &\textbf{474.8}\\
        % $\cos$ + OT (Ensemble model) &\textbf{69.3} &\textbf{91.6} &{95.1} &\textbf{49.8} &\textbf{78.1} &\textbf{85.6} &\textbf{469.5}\\
        % $\cos$ + OT (Ensemble) &{69.0} &{90.7} &{95.7} &\textbf{50.1} &\textbf{78.4} &\textbf{85.6} &\textbf{469.5}\\
        % \hline
        % \hline
        \hline
        \noalign{\smallskip}
        % & \multicolumn{7}{c}{MS-COCO} \\ 
        % \midrule
        % \hline
        % Order-embeddings (VGG) \cite{vendrov2015order} & 23.3 & -- & 84.7 & 31.7 & -- & 74.6 & -- \\ 
        VSE++ (ResNet) \cite{VSE} & 41.3 & -- & 81.2 & 30.3 & -- & 72.4 & -- \\ 
        DPC (ResNet) \cite{zheng2017dual} & 41.2 & 70.5 & 81.1 & 25.3 & 53.4 & 66.4 & 337.9\\ 
        GXN (ResNet) \cite{gu2018look} & 42.0 & -- & 84.7 & 31.7 & -- & 74.6 & -- \\ 
        SCO (ResNet) \cite{huang2018learning} & 42.8 & 72.3 & 83.0 & 33.1 & 62.9 & 75.5 & 369.6 \\ 
        SCAN (Faster R-CNN, ResNet)\cite{SCAN} & 46.4 & 77.4 & 87.2 & 34.4 & 63.7 & 75.7 & 384.8 \\ 
        % SCAN (Ensemble)\cite{SCAN} & {50.4} & {82.2} & {90.0} & {38.6} & {69.3} & {80.4} & 410.9 \\ 
        % \hline
        \textbf{Ours (Faster R-CNN, ResNet)}:\\
        SCAN + WD &{50.2} &{80.1} &{89.5} &{37.9} &{66.8} &{78.1} &{402.6}\\
        SCAN + GWD &{47.2} & {78.3} &{87.5} &{34.9} &{64.4} &{76.3} &{388.6
}\\
        SCAN + GOT &\textbf{50.5} &\textbf{80.2} &\textbf{89.8} &\textbf{38.1} & \textbf{66.8} &\textbf{78.5} &\textbf{403.9}\\
        %$\cos$ + OT (Ensemble) &\textbf{52.1} &\textbf{82.4} &\textbf{90.7} &\textbf{39.1} &{68.2} &{79.2} &\textbf{411.7}\\
        % Dot + OT (single model, m=0.12) &\textbf{69.3} &{91.0} &{95.7} &{48.4} &{77.2} &{84.7} &{466.3}\\
        % Dot + OT (ensembled model) &\textbf{69.3} &\textbf{91.6} &{95.1} &\textbf{49.8} &\textbf{78.1} &\textbf{85.6} &\textbf{469.5}\\
        \bottomrule
    \end{tabular*}
    \vspace{-2mm}
     \caption{\label{table:retrieval} Results on image-text retrieval evaluated on Recall@$K$ (R@$K$). Upper panel: Flickr30K; lower panel: COCO. 
  }
    \vspace{-3mm}
  \end{center}
\end{table*}

==> table/translate.tex <==

\begin{table*}[!t]
    \centering
    \small
    % \resizebox{\textwidth}{!}{
    \begin{tabular}{l c c c c} %{L{5.5cm} l}
    \hline
    {\bf Model}  & {\bf EN-VI uncased} & {\bf EN-VI cased} & {\bf EN-DE uncased} & {\bf EN-DE cased}\\ 
    \hline
    Transformer~\cite{vaswani2017attention}    & $29.25 \pm 0.18$ & $28.46 \pm 0.17$ & $25.60 \pm 0.07$ & $25.12 \pm 0.12$\\
    Transformer + WD  & $29.49 \pm 0.10$ & $28.68 \pm 0.14$ & $25.83 \pm 0.12$ & $25.30 \pm 0.11$\\
    Transformer + GWD & $28.65 \pm 0.14$ & $28.34 \pm 0.16$ & $25.42 \pm 0.17$ & $24.82 \pm 0.15$\\
    Transformer + GOT & $\mathbf{29.92 \pm 0.11}$ & $\mathbf{29.09 \pm 0.18}$ & $\mathbf{26.05 \pm 0.17}$ & $\mathbf{25.54 \pm 0.15}$\\
    \hline
    \end{tabular}
    % }
    \vspace{-2mm}
    \caption{\label{tab:mt} Results of neural machine translation on EN-DE and EN-VI.}
    %\vspace{-3mm}
\end{table*}


==> table/translate_ablation.tex <==

\begin{table}[t]
    \centering
    \small
    % \resizebox{\textwidth}{!}{
    \begin{tabular}{l c c } %{L{5.5cm} l}
    \hline
    {\bf Model}  & {\bf EN-VI uncased} & {\bf EN-DE uncased} \\ 
    \hline
    GOT (shared) & ${29.92 \pm 0.11}$ & ${26.05 \pm 0.18}$  \\
    GOT (unshared) & ${29.77 \pm 0.12}$ & ${25.89 \pm 0.17}$  \\
    \hline
    \end{tabular}
    % }
    \caption{\label{tab:mt_ablation_shareT} Ablation study on transport plan in machine translation. Both models were run 5 times with the same hyper-parameter setting.}
\end{table}


==> table/translate_lambda_ablation.tex <==

%\begin{table}[!t]
%    \centering
%    \small
%%    %\resizebox{0.48\textwidth}{!}{
%    \begin{tabular}{l c c c c c} %{L{5.5cm} l}
%    \hline
%    {\bf Model}  & {\bf BUTD} & {\bf BAN} & {\bf BAN+GW} & {\bf BAN+W} & {\bf BAN+GOT}\\ 
%    \hline
%    
%    {\bf Score} & $63.37$ & $66.00$ & $66.21$ & $66.26$ & $66.44$\\
%
%    \hline
%    \end{tabular}
%    %}
%    \caption{\label{tab:vqa} Results on VQA 2.0 validation set. \cite{kim2018bilinear}}
%    \vspace{-3mm}
%\end{table}

\begin{table}[!t]
    \centering
    \small
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{l c  c c c c c} %{L{5.5cm} l}
    \hline
    {\bf $\lambda$}  & 0  & 0.1 & 0.3 & 0.5 & 0.8 & 1.0\\ 
    \hline
    
    {\bf BLEU} & $28.65$  & $29.31$ & $29.52$ & $29.65$ & {\bf 29.92} & $29.49$\\

    \hline
    \end{tabular}
    }
    \vspace{-3mm}
    \caption{\label{tab:lambda_ab} Ablation study of the hyper-parameter $\lambda$ on the EN-VI machine translation dataset.}
    \vspace{-3mm}
\end{table}


==> table/vqa_ban.tex <==

%\begin{table}[!t]
%    \centering
%    \small
%%    %\resizebox{0.48\textwidth}{!}{
%    \begin{tabular}{l c c c c c} %{L{5.5cm} l}
%    \hline
%    {\bf Model}  & {\bf BUTD} & {\bf BAN} & {\bf BAN+GW} & {\bf BAN+W} & {\bf BAN+GOT}\\ 
%    \hline
%    
%    {\bf Score} & $63.37$ & $66.00$ & $66.21$ & $66.26$ & $66.44$\\
%
%    \hline
%    \end{tabular}
%    %}
%    \caption{\label{tab:vqa} Results on VQA 2.0 validation set. \cite{kim2018bilinear}}
%    \vspace{-3mm}
%\end{table}

\begin{table}[!t]
    \centering
    \small
    %\resizebox{0.48\textwidth}{!}{
    \begin{tabular}{l c c c c} %{L{5.5cm} l}
    \hline
    {\bf Model}  &  {\bf BAN} & {\bf BAN+GWD} & {\bf BAN+WD} & {\bf BAN+GOT}\\ 
    \hline
    
    {\bf Score} & 66.00 & 66.21 & 66.26 & \textbf{66.44}\\

    \hline
    \end{tabular}
    %}
    \vspace{-3mm}
    \caption{\label{tab:vqa} Results (accuracy) on VQA 2.0 validation set, using BAN~\cite{kim2018bilinear} as baseline.}
    %\vspace{-2mm}
\end{table}

